Solving Stochastic Optimization by Newton-type methods with Dimension-Adaptive Sparse Grid Quadrature

Stochastic optimisation problems minimise expectations of random cost functions. We use 'optimise then discretise' method to solve stochastic optimisation. In our approach, accurate quadrature methods are required to calculate the objective, gradient or Hessian which are in fact integrals. We apply the dimension-adaptive sparse grid quadrature to approximate these integrals when the problem is high dimensional. Dimension-adaptive sparse grid quadrature shows high accuracy and efficiency in computing an integral with a smooth integrand. It is a kind of generalisation of the classical sparse grid method, which refines different dimensions according to their importance. We show that the dimension-adaptive sparse grid quadrature has better performance in the optimise then discretise' method than the 'discretise then optimise' method.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{mathrsfs}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{The combination technique applied to the computation of quantities of interest}
\newcommand{\RunningTitle}{The combination of quantities of interest}
\newcommand{\TheAuthors}{B.~Harding, M.~Heland, F.~Huber, Y.~Zhou}

% Sets running headers as well as PDF title and authors
%\headers{\TheTitle}{\TheAuthors}
\headers{\RunningTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors DATE.
\funding{This work was funded by $\dots$}}}

% Authors: full names plus addresses.
\author{
  Brendan Harding\thanks{The Australian National University, Canberra, Australia
    (\email{brendan.harding@anu.edu.au} ).}%, \url{http://www.imag.com/\string~ddoe/}).}
  \and
  Markus Hegland\thanks{The Australian National University, Canberra, Australia
    (\email{markus.hegland@anu.edu.au} ).}
  \and
  Felix Huber\thanks{University of Stuttgart, Stuttgart, Germany
    (\email{fh-stein@web.de} ).}
  \and
  Yuancheng Zhou\thanks{The Australian National University, Canberra, Australia
    (\email{yuancheng.zhou@anu.edu.au} ).}
}

\usepackage{amsopn}
%\DeclareMathOperator{\diag}{diag}
\newcommand{\mi}[1]{\underline{#1}}
\newcommand{\Q}{\mathcal{Q}}


% v~~ REMOVE THE TODONOTES PACKAGE ~~v
\usepackage{xargs}[2008/03/08]
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
% ^~~                              ~~^

\global\long\def\d#1{\,\mathrm{d}#1}
\global\long\def\dd#1#2{\,\mathrm{d}#1\mathrm{d}#2}
\global\long\def\dx{\d x}
\global\long\def\dxy{\dd xy}
\global\long\def\for{\qquad\text{for }}
\global\long\def\v#1{\mathbf{#1}} %vectors
\global\long\def\m#1{\vec{\mathbf{#1}}} %multiindices
\global\long\def\O#1{\mathcal{O}\negmedspace\left(#1\right)}
\global\long\def\eq{={}}
\global\long\def\period{\text{.}}
\global\long\def\e{\mathrm{e}}
\global\long\def\nicefrac#1#2{\frac{#1}{#2}} % TODO how do I get these? Or are they bad style?
\global\long\def\coloneqq{:=} % or shall we use the mathtools package?
\global\long\def\eqqcolon{=:}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:

